B-fields In STar-forming Region Observations (BISTRO): Technical Foundations for Quantitative 450/850 $\mu$m JCMT SCUBA-2/POL-2 Polarimetry

We present five technical validations of SCUBA-2/POL-2 polarimetry on the James Clerk Maxwell Telescope at 450 and 850 $\mu$m, using 174 archival fields in 69 molecular cloud regions and subsets appropriate to each test. Extended-source calibration avoids a deterministic shift of $\Delta\beta=-1.05$ in the dust emissivity index $\beta$ that would result from calibrating extended emission using peak brightness. We modeled Stokes $I$ noise with additive and signal-dependent components. The measured median ratio of surface-brightness noise at 450/850 $\mu$m is 25. Independent tests of Stokes $Q,U$ noise support approximately equal additive variances and weak error correlations, providing a basis for propagating polarization uncertainties. Corrections determined for individual fields reduce additive zero-level offsets of order $1$ mJy arcsec$^{-2}$ in the 450 $\mu$m Stokes $Q$ and $U$ intensities. The three-step regression leaves a median combined residual amplitude of $0.07$ mJy arcsec$^{-2}$. Independent comparisons with SOFIA/HAWC+ at 154 and 214 $\mu$m support the correction in strongly affected fields. We matched the 450 $\mu$m maps to the modeled 850 $\mu$m beam and the common $12.6''$-$300''$ range of angular scales. We compared three reductions of the same 450 $\mu$m observations across 30 sources. Taking the median angular residual relative to the final product for each source, we find that beam matching reduces the median over sources from $6.3^\circ$ to $4.7^\circ$. After matching, 29 of the 30 sources have median residuals below $10^\circ$. We also quantified how residual $Q/U$ offsets propagate in ratios of polarization fractions, differences in spectral indices, and polarization angles. These validations provide procedures and quantitative references for interpreting POL-2 measurements and combining them with polarimetry at other wavelengths.

==> xref_frozen_T_pasj.tex <==
\makeatletter
\newlabel{S1-sec:obs}{{2}{9}{}{section.\theH@article .2}{}}
\newlabel{S1-sec:results}{{3}{13}{}{section.\theH@article .3}{}}
\newlabel{S1-ss:Iratio}{{3.3}{17}{}{subsection.\theH@article .3}{}}
\newlabel{S1-ss:P_ratio}{{3.2}{14}{}{subsection.\theH@article .2}{}}
\newlabel{S1-ss:S_dispersion}{{3.5}{20}{}{subsection.\theH@article .5}{}}
\newlabel{S1-ss:SpIdx}{{3.4}{17}{}{subsection.\theH@article .4}{}}
\newlabel{S1-ss:bfield_consistency}{{3.1}{13}{}{subsection.\theH@article .1}{}}
\newlabel{S1-tbl:S1_dependency}{{3}{10}{}{table.\theH@article .3}{}}
\newlabel{S2-afig:Bmap_B211MO}{{22}{86}{}{figure.\theH@article .22}{}}
\newlabel{S2-afig:Bmap_DR21DR}{{65}{129}{}{figure.\theH@article .65}{}}
\newlabel{S2-afig:Bmap_GC20KC}{{80}{144}{}{figure.\theH@article .80}{}}
\newlabel{S2-afig:Bmap_GCBRCK}{{81}{145}{}{figure.\theH@article .81}{}}
\newlabel{S2-afig:Bmap_GSGRB2}{{87}{151}{}{figure.\theH@article .87}{}}
\newlabel{S2-afig:Bmap_IC139E}{{60}{124}{}{figure.\theH@article .60}{}}
\newlabel{S2-afig:Bmap_MonoR2}{{57}{121}{}{figure.\theH@article .57}{}}
\newlabel{S2-afig:Bmap_N133MO}{{34}{98}{}{figure.\theH@article .34}{}}
\newlabel{S2-afig:Bmap_N633MO}{{69}{133}{}{figure.\theH@article .69}{}}
\newlabel{S2-afig:Bmap_OphiuA}{{24}{88}{}{figure.\theH@article .24}{}}
\newlabel{S2-afig:Bmap_OphiuC}{{26}{90}{}{figure.\theH@article .26}{}}
\newlabel{S2-afig:Bmap_OriAS1}{{37}{101}{}{figure.\theH@article .37}{}}
\newlabel{S2-afig:Bmap_RoseMO}{{67}{131}{}{figure.\theH@article .67}{}}
\newlabel{S2-afig:Bmap_SD24P4}{{44}{108}{}{figure.\theH@article .44}{}}
\newlabel{S2-afig:Bmap_SerpMO}{{43}{107}{}{figure.\theH@article .43}{}}
\newlabel{S2-app:distance}{{5}{79}{}{section.\theH@article .5}{}}
\newlabel{S2-eq:planck_correction}{{9}{33}{}{equation.\theH@article .9}{}}
\newlabel{S2-fig:SpIdx_maps_OphA}{{6}{35}{}{figure.\theH@article .6}{}}
\newlabel{S2-sec:S2_results}{{3}{12}{}{section.\theH@article .3}{}}
\newlabel{S2-ss:S2_HGBS}{{3.6}{51}{}{subsection.\theH@article .6}{}}
\newlabel{S2-ss:S2_P_ratio}{{3.3}{22}{}{subsection.\theH@article .3}{}}
\newlabel{S2-ss:S2_SpIdx}{{3.4}{32}{}{subsection.\theH@article .4}{}}
\newlabel{S2-sss:SpIdxFramework}{{3.4.1}{32}{}{subsubsection.\theH@article .1}{}}
\newlabel{S2-sss:SpIdx_Global}{{3.4.3}{34}{}{subsubsection.\theH@article .3}{}}
\newlabel{S2-sss:SpIdx_OphA}{{3.4.2}{34}{}{subsubsection.\theH@article .2}{}}
\newlabel{S2-tab:surv}{{19}{81}{}{table.\theH@article .19}{}}
\newlabel{S2-tbl:S2_dependency}{{3}{13}{}{table.\theH@article .3}{}}
\newlabel{S2-tbl:SpIdx_Global}{{7}{40}{}{table.\theH@article .7}{}}
\makeatother

